Diversify, Don't Fine-Tune: Scaling Up Visual Recognition Training with Synthetic Images

Recent advances in generative deep learning have enabled the creation of high-quality synthetic images in text-to-image generation. Prior work shows that fine-tuning a pretrained diffusion model on ImageNet and generating synthetic training images from the finetuned model can enhance an ImageNet classifier's performance. However, performance degrades as synthetic images outnumber real ones. In this paper, we explore whether generative fine-tuning is essential for this improvement and whether it is possible to further scale up training using more synthetic data. We present a new framework leveraging off-the-shelf generative models to generate synthetic training images, addressing multiple challenges: class name ambiguity, lack of diversity in naive prompts, and domain shifts. Specifically, we leverage large language models (LLMs) and CLIP to resolve class name ambiguity. To diversify images, we propose contextualized diversification (CD) and stylized diversification (SD) methods, also prompted by LLMs. Finally, to mitigate domain shifts, we leverage domain adaptation techniques with auxiliary batch normalization for synthetic images. Our framework consistently enhances recognition model performance with more synthetic data, up to 6x of original ImageNet size showcasing the potential of synthetic data for improved recognition models and strong out-of-domain generalization.

==> tables/bn.tex <==
%!TEX root = ../main.tex

\begin{table}[h!]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lccc}
\toprule
 & \textbf{ResNet-50} & \textbf{ResNet-101} & \textbf{ResNet-152} \\
\hline
Vanilla BN & 78.32 & 79.92 & 80.43 \\
Separate BN & \textbf{78.93} & \textbf{80.34} & \textbf{81.05} \\
\bottomrule
\end{tabular}
}
\caption{\textbf{Vanilla \vs Separate BN}. Results are generated with 2.4M synthetic images with diversification. Separate BN is demonstrated to be effective for training on real+synthetic data, across various model architectures. }
\label{tab:bn}
\end{table}


==> tables/transfer.tex <==
\begin{table*}[t]
  \centering
  \resizebox{\linewidth}{!}{%
  \begin{tabular}{l|c|c|cccccc|cccccc}
  \toprule
  \multirow{2}{*}{Model} & \multirow{2}{*}{Dataset} & \multirow{2}{*}{Epoch} & \multicolumn{6}{c|}{\textbf{1}$\boldsymbol{\times}$ Schedule} & \multicolumn{6}{c}{\textbf{2}$\boldsymbol{\times}$ Schedule} \\
    & & & AP$^\text{bb}$ & AP$_\text{50}^\text{bb}$  & AP$_\text{75}^\text{bb}$ & AP$^\text{mk}$  & AP$_\text{50}^\text{mk}$  & AP$_\text{75}^\text{mk}$  & AP$^\text{bb}$  & AP$_\text{50}^\text{bb}$  & AP$_\text{75}^\text{bb}$ & AP$^\text{mk}$  & AP$_\text{50}^\text{mk}$  & AP$_\text{75}^\text{mk}$  \\
  \midrule
  ResNet-50 & ImageNet-1k & 130 & 38.2 & 58.1 & 41.2 & 33.3 & 54.7 & 35.2 & 40.0 & 59.9 & 43.1 & 34.7 & 56.5 & 36.9 \\
  ResNet-50 (Ours) & ImageNet-1k + Syn(12M)  & 130 & \textbf{38.8} & 58.7 & 42.0 & \textbf{33.9} & 55.3 & 35.8 & \textbf{40.3} & 60.0 & 43.7 & \textbf{35.1} & 57.0 & 37.0  \\
  ResNet-50 (Ours) & ImageNet-1k + Syn(12M)  & 400 & \textbf{39.0} & 58.3 & 42.6 & \textbf{34.3} & 55.8 & 36.1 & \textbf{40.9} & 60.4 & 44.0 & \textbf{35.8} & 57.0 & 37.3  \\
  \midrule
  ResNet-101 & ImageNet-1k & 200 & 41.4 & 59.6 & 42.7 & 35.4 & 56.5 & 38.1 & 41.3 & 61.3 & 45.0 & 37.3 & 58.3 & 40.3 \\
  ResNet-101 (Ours) & ImageNet-1k + Syn(12M)  & 200 & \textbf{41.9} & 60.0 & 43.9 & \textbf{36.1} & 57.2 & 38.4 & \textbf{41.8} & 61.9 & 45.5 & \textbf{37.9} & 58.4 & 41.2  \\
  ResNet-101 (Ours) & ImageNet-1k + Syn(12M)  & 400 & \textbf{42.4} & 60.5 & 43.7 & \textbf{36.4} & 57.5 & 39.1 & \textbf{42.3} & 62.3 & 46.0 & \textbf{38.3} & 59.3 & 41.3  \\
  \midrule
  ResNet-152 & ImageNet-1k & 200 & 42.7 & 59.9 & 43.1 & 36.2 & 57.8 & 38.5 & 43.1 & 62.1 & 45.7 & 38.6 & 59.1 & 41.3 \\
  ResNet-152 (Ours) & ImageNet-1k + Syn(12M)  & 200 & \textbf{43.2} & 60.3 & 43.8 & \textbf{36.9} & 58.7 & 39.1 & \textbf{43.7} & 62.5 & 46.1 & \textbf{38.9} & 59.5 & 41.8  \\
  ResNet-152 (Ours) & ImageNet-1k + Syn(12M)  & 400 & \textbf{44.0} & 61.2 & 44.0 & \textbf{37.8} & 59.8 & 39.7 & \textbf{44.5} & 63.3 & 46.5 & \textbf{39.8} & 60.3 & 42.3  \\

  \bottomrule
  \end{tabular}}
  \caption{\textbf{Transfer Learning Results on MS COCO}. We use Mask-RCNN with different backbones for evaluation. We report AP for both bounding box and mask predictions of models trained with 1x and 2x schedule. \yj{be consistent in bolding -- i.e., bold all numbers that are best in each column.}}
  \label{tab:detection}
\end{table*}
